Development of a central-moment phase-field lattice Boltzmann model for thermocapillary flows: Droplet capture and computational performance

This study develops a computationally efficient phase-field lattice Boltzmann model with the capability to simulate thermocapillary flows. The model was implemented into the open-source simulation framework, waLBerla, and extended to conduct the collision stage using central moments. The multiphase model was coupled with both a passive-scalar thermal LB, and a RK solution to the energy equation in order to resolve temperature-dependent surface tension phenomena. Various lattice stencils (D3Q7, D3Q15, D3Q19, D3Q27) were tested for the passive-scalar LB and both the second- and fourth-order RK methods were investigated. There was no significant difference observed in the accuracy of the LB or RK schemes. The passive scalar D3Q7 LB discretisation tended to provide computational benefits, while the second order RK scheme is superior in memory usage. This paper makes contributions relating to the modelling of thermocapillary flows and to understanding the behaviour of droplet capture with thermal sources analogous to thermal tweezers. Four primary contributions to the literature are identified. First, a new 3D thermocapillary, central-moment phase-field LB model is presented and implemented in the open-source software, waLBerla. Second, the accuracy and computational performance of various techniques to resolve the energy equation for multiphase, incompressible fluids is investigated. Third, the dynamic droplet transport behaviour in the presence of thermal sources is studied and insight is provided on the potential ability to manipulate droplets based on local domain heating. Finally, a concise analysis of the computational performance together with near-perfect scaling results on NVIDIA and AMD GPU-clusters is shown. This research enables the detailed study of droplet manipulation and control in thermocapillary devices.

==> figures/droplet_migration/droplet_schemantic3DSetup3.tex <==
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
	
	\draw [draw opacity=1 ][line width=3]    (23,16) -- (653,15) ;
	\draw [draw opacity=1 ][line width=3]    (23.5,290) -- (653,289) ;
	
	\draw [draw opacity=1, line width=2, stealth-stealth] (23,305.99) -- (653,304.01) ;
	\draw[draw opacity=1, line width=2, stealth-stealth]   (30.02,16) -- (30,290) ;
	
	\draw[draw opacity=1, line width=2, -stealth]   (50,270) -- (50,170) ;
	\draw[draw opacity=1, line width=2, -stealth]   (40,260) -- (140,260) ;
	
	\draw[draw opacity=1, line width=2]   (232,137) -- (200,137) ;
	
	
	\filldraw[color=gray!60, fill=gray!5, very thick](200,137) circle (32);
	
	\draw[draw opacity=1, line width=1]   (232,137) -- (200,137) ;
	
	
	
	\foreach \r in {4, 12, 20, 28, 36}
	{
		\draw[color=red!60, very thick](400,158) circle (\r);
	}
	
	\foreach \r in {4, 12, 20, 28, 36}
	{
		\draw[color=red!60, very thick](400,116) circle (\r);
	}
	
	
	
	% Text Node
	
	\draw (326,310.4) node [anchor=north west][inner sep=0.75pt]    {$L$};
	% Text Node
	\draw (40,90.4) node [anchor=north west][inner sep=0.75pt]    {$B$};
	% Text Node
	\draw (135,265) node [anchor=north west][inner sep=0.75pt]    {$x$};
	% Text Node
	\draw (35,170) node [anchor=north west][inner sep=0.75pt]    {$z$};
	
	\draw (210,125) node [anchor=north west][inner sep=0.75pt]    {$R$};
	\draw (172,140) node [anchor=north west][inner sep=0.75pt]    {$(x_c, y_c, z_c)$};
	
	
	
\end{tikzpicture}
